SpectraNet: Learned Recognition of Artificial Satellites From High Contrast Spectroscopic Imagery

Effective space traffic management requires positive identification of artificial satellites. Current methods for extracting object identification from observed data require spatially resolved imagery which limits identification to objects in low earth orbits. Most artificial satellites, however, operate in geostationary orbits at distances which prohibit ground based observatories from resolving spatial information. This paper demonstrates an object identification solution leveraging modified residual convolutional neural networks to map distance-invariant spectroscopic data to object identity. We report classification accuracies exceeding 80% for a simulated 64-class satellite problem--even in the case of satellites undergoing constant, random re-orientation. An astronomical observing campaign driven by these results returned accuracies of 72% for a nine-class problem with an average of 100 examples per class, performing as expected from simulation. We demonstrate the application of variational Bayesian inference by dropout, stochastic weight averaging (SWA), and SWA-focused deep ensembling to measure classification uncertainties--critical components in space traffic management where routine decisions risk expensive space assets and carry geopolitical consequences.

==> old_authors.tex <==



\author{J. Zachary Gazak\\
United States Space Force Space Systems Command\\
Kihei, HI 96753\\
{\tt\small jonathan.gazak.1.ctr@us.af.mil}
% For a paper whose authors are all at the same institution,
% omit the following lines up until the closing ``}''.
% Additional authors and addresses can be added with ``\and'',
% just like the second author.
% To save space, use either the email address or home page, not both
\and
Ian McQuaid\\
Air Force Research Lab\\
Kihei, HI 96753\\
{\tt\small ian.mcquaid@centauricorp.com}

\and
Justin Fletcher\\
{\tt\small justin.fletcher.14.ctr@us.af.mil}

\and
Ryan Swindle\\
{\tt\small thomas.swindle.2.ctr@us.af.mil}

\and
Matthew Phelps\\
{\tt\small matthew.phelps.15.ctr@us.af.mil}

United States Space Force Space Systems Command
Kihei, HI 96753\\
}

